The Theory of the Interleaving Distance on Multidimensional Persistence Modules

In 2009, Chazal et al. introduced $\epsilon$-interleavings of persistence modules. $\epsilon$-interleavings induce a pseudometric $d_I$ on (isomorphism classes of) persistence modules, the interleaving distance. The definitions of $\epsilon$-interleavings and $d_I$ generalize readily to multidimensional persistence modules. In this paper, we develop the theory of multidimensional interleavings, with a view towards applications to topological data analysis. We present four main results. First, we show that on 1-D persistence modules, $d_I$ is equal to the bottleneck distance $d_B$. This result, which first appeared in an earlier preprint of this paper, has since appeared in several other places, and is now known as the isometry theorem. Second, we present a characterization of the $\epsilon$-interleaving relation on multidimensional persistence modules. This expresses transparently the sense in which two $\epsilon$-interleaved modules are algebraically similar. Third, using this characterization, we show that when we define our persistence modules over a prime field, $d_I$ satisfies a universality property. This universality result is the central result of the paper. It says that $d_I$ satisfies a stability property generalizing one which $d_B$ is known to satisfy, and that in addition, if $d$ is any other pseudometric on multidimensional persistence modules satisfying the same stability property, then $d\leq d_I$. We also show that a variant of this universality result holds for $d_B$, over arbitrary fields. Finally, we show that $d_I$ restricts to a metric on isomorphism classes of finitely presented multidimensional persistence modules.

==> R_Computation.tex <==
\section{Computation of $d_I$ is Equivalent to Deciding Solvability of Quadratics}\label{ComputationSection}

\subsection{Overview}
Let ${\mathcal MQ}(k)$ denote the set of multivariate systems of quadratic equations over the field $k$.

We show in this section (Theorem~\ref{InterleavingAndQuadratics}) that, given finite presentations for $n$-modules $M$ and $N$, for any $\epsilon>0$ deciding whether $M$ and $N$ are $\epsilon$-interleaved is polynomially equivalent to deciding the solvability of an instance $Q(M,N,\epsilon)$ of ${\mathcal MQ}(k)$ with $O(m^2)$ unknowns and $O(m^2)$ equations, where $q$ is the total number of generators and relations in the presentations for $M$ and $N$.

We also show (Proposition~\ref{PossibilitiesForInterleavingDistance}) that $d_I(M,N)$ must be equal to one of the elements of an order $O(m^2)$ subset of $[0,\infty)$ defined in terms of the grades of generators and relations of $M$ and $N$.  Thus, by searching through this subset, we can compute $d_I(M,N)$ by deciding whether $Q(M,N,\epsilon)$ has a solution for $O(\log m)$ values of $\epsilon$.  Thus we can compute $d_I(M,N)$ by deciding the solvability of $O(\log m)$ instances of ${\mathcal MQ}(k)$.

In fact, computing $d_I(M,N)$ is equivalent to deciding the solvability of these $O(\log q)$ instances of ${\mathcal MQ}(k)$; after all, if $d_I(M,N)=\epsilon$ then by the Closure Theorem (Theorem~\ref{InterleavingThm}), $M$ and $N$ are $\epsilon'$-interleaved if and only if $\epsilon'\geq \epsilon$.  Thus for all $\epsilon'\geq 0$, the value of $d_I$ determines whether $Q(M,N,\epsilon')$ has a solution.

We state this result as a theorem:

\begin{thm}[Characterization of Computation of $d_I$]\label{Thm:ComputationResult}
Given finite presentations for two multidimensional persistence modules $M$ and $N$, the problem of computing $d_I(M,N)$ is polynomially equivalent to deciding the solvability of $O(\log m)$ instances of ${\mathcal MQ}(k)$, each with $O(m^2)$ variables and $O(m^2)$ equations, where $m$ is the total number of generators and relations in the presentations for $M$ and $N$.
\end{thm}
%
The rest of this section is devoted to the statement and proof of Theorem~\ref{InterleavingAndQuadratics} and Proposition~\ref{PossibilitiesForInterleavingDistance}.

%If $k$ is a field of prime order, a standard algorithm based on Gr\"obner bases determines the solvability of systems in ${\mathcal MQ}(k)$.  ${\mathcal MQ}(k)$ is NP-complete, however, and this algorithm is for general instances of ${\mathcal MQ}(k)$ prohibitively inefficient.  We leave it to future work to investigate the complexity and tractability in practice of deciding the solvability of the systems of quadratics $Q(M,N,\epsilon)$ arising in our reduction.

%\paragraph{A Word on Minimal Presentations}
%MOVE
%In practice, we are interested in computing $d_I$ between the persistent homology modules of two simplicial $n$-filtrations.  To apply our reduction to this problem, we would need a way of computing a presentation of the persistent homology module of a simplicial $n$-filtration; strictly speaking, our reduction would not require that the presentations of our modules be minimal.  However, to minimize the number and size of the quadratic systems we would need to consider in computing the interleaving distance via this reduction, we would want the presentations we compute to be minimal.
%
%The problem of computing minimal presentations of multidimensional persistence modules also seems to be of interest, independent of potential applications to computing $d_I$; minimal presentations are maximally compact ways of representing persistence modules, and as such, I imagine that a minimal presentations could be suitable inputs for a variety of computations involving multidimensional persistence modules.  
%
%The computational commutative algebra community has studied variants of this problem \cite{} and has developed tools that could be useful in the TDA setting \cite{}; see also \cite{}.  

%We hope to address the problem of computing a minimal presentation of the persistent homology module of a simplicial $n$-filtration in future work. 

\subsection{Linear Algebraic Representations of Homogeneous Elements and Morphisms of Free $n$-Modules}

\subsubsection{Representing Homogeneous Elements of Free $n$-Modules as Vectors}\label{HomogeneousEltsAsVectors}
Given a finitely generated free $n$-module $F$ and an (ordered) basis $B=b_1,\ldots,b_l$ for $F$, we can represent a homogeneous element $v\in F$ as a pair $([v,B],\gr(v))$ where $[v,B]\in k^l$ is a vector: if $v=\sum_{i:\gr(v)\geq \gr(b_i)} a_i \varphi_F(\gr(b_i),\gr(v))(b_i)$, with each $a_i\in k$, then for $1\leq i\leq l$ we define 
\[[v,B]_i=
\begin{cases}
a_i &\text{if }\gr(v)\geq \gr(b_i)\\
0 &\text{otherwise.} 
\end{cases}
\]

\begin{remark}\label{StandardBasisRemark} Note that for $1\leq i\leq l$, $[b_i,B]=\e_i$, where $\e_i$ denotes the $i^{\th}$ standard basis vector in $k^l$. \end{remark}

If $V\subset F$ is a homogeneous set, we define $[V,B]=\{[v,B]|v\in V\}$. 

\subsubsection{Representing Morphisms of $n$-Modules as Matrices}
Given finitely generated free $n$-modules $F$ and $F'$ and (ordered) bases $B=b_1,\ldots,b_l$ and $B'=b'_1,\ldots,b'_m$ for $F$ and $F'$ respectively, let $\Mat_k(B,B')$ denote the set of $m\times l$ matrices $A$ with entries in $k$ such that $A_{ij}=0$ whenever $\gr(b_j)<\gr(b'_i)$.

We can represent any $f\in\hom(F,F')$ as a matrix $[f,B,B']\in \Mat_k(B,B')$, where if $f(b_j)=\sum_{i:\gr(b_j)\geq \gr(b'_i)} a_{ij} \varphi_{F'}(\gr(b'_i),\gr(b_j))(b'_i)$, with each $a_{ij}\in k$, then 
\[[f,B,B']_{ij}=
\begin{cases}
a_{ij} &\text{if }\gr(b_j)\geq \gr(b'_i)\\
0 &\text{otherwise.} 
\end{cases}
\]
%
\begin{lem}\label{MatrixRepBijectionLemma} The map $[\cdot,B,B']:\hom(F,F')\to \Mat_k(B,B')$ is a bijection.\end{lem}
\begin{proof} The proof is straightforward.\end{proof}
Note also the following additional properties of these matrix representations of morphisms between free $n$-modules:
%
\begin{lem}\label{MatrixRepProperties} Let $F,F',F''$ be free $n$-modules with ordered bases $B,B',B''$.  
\begin{enumerate*}
%\item For $v\in F$ homogeneous and $f\in \hom(F,F')$, $[f(v),B']=[f,B,B'][v,B]$, 
\item[(i)]If $f_1,f_2\in \hom(F,F')$ then $[f_1+f_2,B,B']=[f_1,B,B']+[f_2,B,B']$,
\begin{sloppypar}
\item[(ii)]If $f_1\in \hom(F,F')$, $f_2\in \hom(F',F'')$ then $[f_2\circ f_1,B,B'']=[f_2,B',B''][f_1,B,B']$,
\end{sloppypar}
\item[(iii)]For any $\epsilon\geq 0$, $[\varphi_{F}(\epsilon),B,B(\epsilon)]=I_{|B|}$, where for $m\in {\mathbb N}$, $I_m$ denotes the $m\times m$ identity matrix.
\end{enumerate*}
\end{lem}
\begin{proof} The proof of each of these results is straightforward. \end{proof}

For a graded set $W$ and $u\in \R^n$, let $W^u=\{y\in W|\gr(y)\leq u\}$.

\begin{lem}\label{MappingIntoSubModLemma} If $F_1$,$F_2$ are free $n$-modules with bases $B_1$,$B_2$ and $W_1\subset F_1$,$W_2\subset F_2$ are sets of homogeneous elements then a morphism $f:F_1\to F_2$ maps $\free[W_1]$ into $\free[W_2]$ iff $[f,B_1,B_2][w,B_1]\in \newspan[W_2^{\gr(w)},B_2]$ for every $w\in W_1$. 
\end{lem}      

\begin{proof} %This follows from the first result of Lemma~\ref{MatrixRepProperties}. 
This is straightforward.  
\end{proof}

\subsection{Finitely Presented $n$-Modules are $\epsilon$-Interleaved iff a Quadratic Has a Solution}

Let $\langle G_M|R_M \rangle$, $\langle G_N|R_N \rangle$ be presentations for finitely presented $n$-modules $M$ and $N$, and assume the elements of each of the sets $G_M,G_N,R_M,R_N$ are endowed with a total order, which may be chosen arbitrarily.  For a finite ordered set $T$ and $1\leq i\leq |T|$, let $T_{,i}$ denote the $i^{\th}$ element of $T$.

We now define six matrices of variables, each with some of the variables constrained to be 0.  Namely, we define
\begin{itemize*}
\item ${\mathbf A}$, a $|G_N|\times |G_M|$ matrix of variables with ${\mathbf A}_{ij}=0$ if $\gr(G_{M,j})+\vec\epsilon\not\geq \gr(G_{N,i})$. 
\item ${\mathbf B}$, a $|G_M|\times |G_N|$ matrix of variables with ${\mathbf B}_{ij}=0$ if $\gr(G_{N,j})+\vec\epsilon\not\geq \gr(G_{M,i})$.
\item ${\mathbf C}$, an $|R_N|\times |R_M|$ matrix of variables with ${\mathbf C}_{ij}=0$ if $\gr(R_{M,j})+\vec\epsilon\not\geq \gr(R_{N,i})$.
\item ${\mathbf D}$, an $|R_M|\times |R_N|$ matrix of variables with ${\mathbf D}_{ij}=0$ if $\gr(R_{N,j})+\vec\epsilon\not\geq \gr(R_{M,i})$.
\item ${\mathbf E}$, an $|R_M|\times |G_M|$ matrix of variables with ${\mathbf E}_{ij}=0$ if $\gr(G_{M,j})+2\vec\epsilon\not\geq \gr(R_{M,i})$.
\item ${\mathbf F}$, an $|R_N|\times |G_N|$ matrix of variables with ${\mathbf F}_{ij}=0$ if $\gr(G_{N,j})+2\vec\epsilon\not\geq \gr(R_{N,i})$.
\end{itemize*}

Let $T_M$ denote the $|G_M|\times|R_M|$ matrix whose $i^{\th}$ column is $[R_{M,i},G_M]$ and let $T_N$ denote the $|G_N|\times|R_N|$ matrix whose $i^{\th}$ column is $[R_{N,i},G_N]$.

\begin{thm}\label{InterleavingAndQuadratics} $M$ and $N$ are $\epsilon$-interleaved iff the multivariate system of quadratic equations $Q(M,N,\epsilon)$, given by
\begin{align*}
{\mathbf A}T_M&=T_N{\mathbf C}\\  
{\mathbf B}T_N&=T_M{\mathbf D}\\ 
\mathbf{BA}-I_{|G_M|}&=T_M{\mathbf E}\\
\mathbf{AB}-I_{|G_N|}&=T_N{\mathbf F},
\end{align*}        
has a solution.
\end{thm}

\begin{proof}

To prove the result, we proceed in three steps.  First, we observe that for any free covers $(F_M,\rho_M)$ and $(F_N,\rho_N)$ of $M$ and $N$, the existence of $\epsilon$-interleaving morphisms between $M$ and $N$ is equivalent to the existence of a pair of morphisms between $F_M$ and $F_N$ having certain properties.  We then note that the existence of such morphisms is equivalent to the existence of two matrices, one in $\Mat_k(G_M,G_N)$ and the other in $\Mat_k(G_N,G_M)$, having certain properties.  Finally, we observe that the existence of such matrices is equivalent to the existence of a solution to $Q(M,N,\epsilon)$.

Let $(F_M,\rho_M)$ and $(F_N,\rho_N)$ be free covers of $M$ and $N$.  
\begin{lem}\label{LiftsOfInterleavingsLemma} $M$ and $N$ are $\epsilon$-interleaved iff there exist morphisms ${\tilde f}:F_M\to F_N(\epsilon)$ and ${\tilde g}:F_N\to F_M(\epsilon)$ such that
\begin{enumerate*}
\item ${\tilde f}(\ker(\rho_M))\subset \ker(\rho_N(\epsilon))$,
\item ${\tilde g}(\ker(\rho_N))\subset \ker(\rho_M(\epsilon))$,
\item ${\tilde g}\circ {\tilde f}-\varphi_{F_M}(2\epsilon)\subset \ker(\rho_M(2\epsilon))$,
\item ${\tilde f}\circ {\tilde g}-\varphi_{F_N}(2\epsilon)\subset \ker(\rho_N(2\epsilon))$.
\end{enumerate*}
\end{lem}
We'll call morphisms ${\tilde f},{\tilde g}$ satisfying the above properties {\bf $\epsilon$-interleaved lifts} of the free covers $(F_M,\rho_M)$ and $(F_N,\rho_N)$.

\begin{proof} Let $f:M\to N(\epsilon)$ and $g:N\to M(\epsilon)$ be interleaving morphisms.  Then by Lemma~\ref{ExistenceAndHomotopyUniquenessOfLifts} there exist lifts ${\tilde f}:F_M \to F_N(\epsilon)$ and ${\tilde g}:F_N\to F_M(\epsilon)$ of $f$ and $g$.  By the definition of a lift, ${\tilde f}$ and ${\tilde g}$ satisfy properties 1 and 2 in the statement of the lemma.  ${\tilde g}\circ {\tilde f}$ is a lift of $g\circ f=\varphi_{M}(2\epsilon)$.  $\varphi_{F_M}(2\epsilon)$ is also a lift of $\varphi_{M}(2\epsilon)$, so by the uniqueness up to homotopy of lifts (Lemma~\ref{ExistenceAndHomotopyUniquenessOfLifts}), ${\tilde f}$ and ${\tilde g}$ satisfy property 3.  The same argument shows that ${\tilde f}$ and ${\tilde g}$ satisfy property 4.

The converse direction is straightforward; we omit the details. 
\end{proof}

Now let $F_M=\free[G_M]$, $F_N=\free[G_N]$, and let $\rho_M:F_M \to F_M/\langle R_M \rangle$, $\rho_N:F_N \to F_N/\langle R_N \rangle$ be the quotient maps.  Since the interleaving distance between two modules is an isomorphism invariant of the modules, we may assume without loss of generality that $F_M/\langle R_M \rangle=M$ and $F_N/\langle R_N \rangle=N$.  Then $(F_M,\rho_M)$ and $(F_N,\rho_N)$ are free covers of $M$ and $N$.    

\begin{sloppypar}
\begin{lem}\label{MatrixLemma} $M$ and $N$ are $\epsilon$-interleaved iff there exist matrices $A\in \Mat_k(G_M,G_N)$ and $B\in \Mat_k(G_N,G_M)$ such that
\begin{enumerate*}
\item $A[w,G_M]\in \newspan [R_N^{\gr(w)+\vec\epsilon},G_N]$ for all $w\in R_M$,
\item $B[w,G_N]\in \newspan [R_M^{\gr(w)+\vec\epsilon},G_M]$ for all $w\in R_N$,
\item $(BA-I_{|G_M|})(\e_i)\in \newspan [R_M^{\gr(G_{M,i})+2\vec\epsilon},G_M]$ for $1\leq i \leq |G_M|$,
\item $(AB-I_{|G_N|})(\e_i)\in \newspan [R_N^{\gr(G_{N,i})+2\vec\epsilon},G_N]$ for $1\leq i \leq |G_N|$.
\end{enumerate*}
\end{lem}
\end{sloppypar}
%We'll call such ${\mathbf A}$ and ${\mathbf B}$ {\bf $\epsilon$-interleaved lift matrices}. 

\begin{proof}
By Lemma~\ref{LiftsOfInterleavingsLemma}, $M$ and $N$ are $\epsilon$-interleaved iff there exists $\epsilon$-interleaved lifts ${\tilde f}:F_M\to F_N$ and ${\tilde g}:F_N\to F_M$ of the free covers $(F_M,\rho_M)$ and $(F_N,\rho_N)$.  

By Lemma~\ref{MappingIntoSubModLemma}, morphisms ${\tilde f}:F_M\to F_N$ and ${\tilde g}:F_N\to F_M$, are $\epsilon$-interleaved lifts iff
\begin{enumerate*}
\item $[{\tilde f},G_M,G_N(\epsilon)][w,G_M]\in \newspan [R_N(\epsilon)^{\gr(w)},G_N(\epsilon)]$ for all $w\in R_M$,
\item $[{\tilde g},G_N,G_M(\epsilon)][w,G_N]\in \newspan [R_M(\epsilon)^{gw(w)},G_M(\epsilon)]$ for all $w\in R_N$,
\item $[{\tilde g}\circ {\tilde f}-\varphi_{F_M}(2\epsilon),G_M,G_M(2\epsilon)][w,G_M]\in \newspan [R_M(2\epsilon)^{\gr(w)},G_M(2\epsilon)]$ for all $w\in G_M$,
\item $[{\tilde f}\circ {\tilde g}-\varphi_{F_N}(2\epsilon),G_N,G_N(2\epsilon)][w,G_N]\in \newspan [R_N(2\epsilon)^{\gr(w)},G_N(2\epsilon)]$ for all $w\in G_N$.
\end{enumerate*}
By Lemma~\ref{MatrixRepProperties}, 

\[[{\tilde g}\circ {\tilde f}-\varphi_{F_M}(2\epsilon),G_M,G_M(2\epsilon)]=[{\tilde g},G_N,G_M(\epsilon)][{\tilde f},G_M,G_N(\epsilon)]-I_{|G_M|}\] 
and
\[[{\tilde f}\circ {\tilde g}-\varphi_{F_N}(2\epsilon),G_N,G_N(2\epsilon)]=[{\tilde f},G_M,G_N(\epsilon)][{\tilde g},G_N,G_M(\epsilon)]-I_{|G_N|}.\]
Also, by Remark~\ref{StandardBasisRemark}, for $1\leq i\leq |G_M|$, $[G_{M,i},G_M]=\e_i$, where $\e_i$ is the $i^{\th}$ standard basis vector in $k^{|G_M|}$.  Similarly, for $1\leq i\leq |G_N|$, $[G_{N,i},G_N]=\e_i$, where $\e_i$ is the $i^{\th}$ standard basis vector in $k^{|G_N|}$.

Finally, note that we have that 
\begin{align*}
[R_N(\epsilon)^{\gr(w)},G_N(\epsilon)]&=[R_N^{\gr(w)+\vec\epsilon},G_N] \text{\rm{ for all }} w\in R_M,\\
[R_M(\epsilon)^{gw(w)},G_M(\epsilon)]&=[R_M^{\gr(w)+\vec\epsilon},G_M] \text{\rm{ for all }} w\in R_N,\\
[R_M(2\epsilon)^{\gr(w)},G_M(2\epsilon)]&=[R_M^{\gr(w)+2\vec\epsilon},G_M] \text{\rm{ for all }} w\in G_M,\\ 
[R_N(2\epsilon)^{\gr(w)},G_N(2\epsilon)]&=[R_N^{\gr(w)+2\vec\epsilon},G_N] \text{\rm{ for all }} w\in G_N. 
\end{align*}

Using all of these observations, Lemma~\ref{MatrixLemma} now follows from Lemma~\ref{MatrixRepBijectionLemma}.
\end{proof}

Finally, Theorem~\ref{InterleavingAndQuadratics} follows from Lemma~\ref{MatrixLemma} by way of elementary matrix algebra and, in particular, the basic fact that for $l,m\in {\mathbb N}$ and vectors $v,v_1,\ldots,v_l$ in $k^m$, $v\in \newspan(v_1,\ldots,v_l)$ iff there exists a vector $w\in k^{l}$ such that $v=V w$, where $V$ is the $m\times l$ matrix whose $i^{\th}$ column is $v_i$.
\end{proof}

\begin{remark}\label{ComputationRemark} Note that each of the number of equations and the number of variables in $Q(M,N,\epsilon)$ is $O(q^2)$, where $q$ is the total number of generators and relations in the presentations for $M$ and $N$.  Note also that $Q(M,N,\epsilon)$ has as few variables and equations as possible when the presentations for $M$ and $N$ are minimal.
\end{remark}

\subsection{Determining Possible Values for $d_I(M,N)$}

Let $M$ and $N$ be finitely presented $n$-modules, and let $U_M^i$, $U_N^i$, $U_M$, and $U_N$ be as defined at the beginning of Section~\ref{Sec:ClosureTheorem}.  Let \[U_{M,N}=\bigcup_i\left( \{|x-y|\}_{x\in U_M^i,y\in U_N^i} \cup \{\frac{1}{2}|x-y|\}_{x,y\in U_M^i} \cup \{\frac{1}{2}|x-y|\}_{x,y\in U_N^i}\right) \cup \{0,\infty\}.\]

Note that $|U_{M,N}|=O(q^2)$, where as above $q$ is the total number of generators and relations in a minimal presentation for $M$ and a minimal presentation for $N$.

\begin{prop}\label{PossibilitiesForInterleavingDistance} $d_I(M,N)\in U_{M,N}$. \end{prop}

\begin{proof} Assume that for some $\epsilon'>0$, $\epsilon'\not\in U_{M,N}$, $M$ and $N$ are $\epsilon'$-interleaved.  Let $\epsilon$ be the largest element of $U_{M,N}$ such that $\epsilon'>\epsilon$, and let $\delta=\epsilon'-\epsilon$.

We'll check that $M,N,\epsilon$ and $\delta$ satisfy the hypotheses of Lemma~\ref{SmallerInterleavingLemma}.  The lemma then implies that $M$ and $N$ are $\epsilon$-interleaved.  The result follows.

By assumption, $M$ and $N$ are $(\epsilon+\delta)$-interleaved, so the first hypothesis of Lemma~\ref{SmallerInterleavingLemma} is satisfied.  We'll show that the second hypothesis is satisfied; the proof that the third hypothesis is satisfied is the same as that for the second hypothesis.

If $z\in U_{M}$ then for no $i$, $1\leq i\leq n$, can an element of $U_N^i$ lie in $(z_i+\epsilon,z_i+\epsilon+\delta]$; if, to the contrary, for some $i$ there were an element $u\in U_N^i\cap(z+\epsilon,z+\epsilon+\delta]$, then we would have $|u-z_i|\in U_{M,N}$, and $\epsilon <|u-z_i|\leq \epsilon+\delta$, which contradicts the way we chose $\epsilon$ and $\delta$.  %$\epsilon'\not\in U_{M,N}$? 
Thus by Lemma~\ref{FirstIsomorphismLemma}, $\varphi_N(z+\epsilon,z+\epsilon+\delta)$ is an isomorphism.

Similarly, for no $i$, $1\leq i\leq n$, can an element of $U_M^i$ lie in $(z_i+2\epsilon,z_i+2\epsilon+2\delta]$; if, to the contrary, for some $i$ there were an element $u\in U_M^i\cap(z+2\epsilon,z+2\epsilon+2\delta]$, then we would have $\frac{1}{2}|u-z_i|\in U_{M,N}$, and $\epsilon <\frac{1}{2}|u-z_i|\leq \epsilon+\delta$, which again contradicts the way we chose $\epsilon$ and $\delta$.  By Lemma~\ref{FirstIsomorphismLemma}, $\varphi_M(z+2\epsilon,z+2\epsilon+2\delta)$ is an isomorphism.

Thus the second hypothesis of Lemma~\ref{SmallerInterleavingLemma} is satisfied by our $M,N,\epsilon$,$\delta$, as we wanted to show. \end{proof}

